Leveraging Large Language Models for Solving Rare MIP Challenges

Mixed Integer Programming (MIP) has been extensively applied in areas requiring mathematical solvers to address complex instances within tight time constraints. However, as the problem scale increases, the complexity of model formulation and finding feasible solutions escalates significantly. In contrast, the model-building cost for end-to-end models, such as large language models (LLMs), remains largely unaffected by problem scale due to their pattern recognition capabilities. While LLMs, like GPT-4, without fine-tuning, can handle some traditional medium-scale MIP problems, they struggle with uncommon or highly specialized MIP scenarios. Fine-tuning LLMs can yield some feasible solutions for medium-scale MIP instances, but these models typically fail to explore diverse solutions when constrained by a low and constant temperature, limiting their performance. In this paper, we propose and evaluate a recursively dynamic temperature method integrated with a chain-of-thought approach. Our findings show that starting with a high temperature and gradually lowering it leads to better feasible solutions compared to other dynamic temperature strategies. Additionally, by comparing results generated by the LLM with those from Gurobi, we demonstrate that the LLM can produce solutions that complement traditional solvers by accelerating the pruning process and improving overall efficiency.

==> sections/3modeling.tex <==
\section{mathematical modeling}
\label{sec:modeling}

Given that LLMs have been trained on numerous traditional MIP problems, such as the TSP, knapsack problem, and more, we aim to assess the robustness of LLMs in MIP by constructing a carpooling MIP model and developing a simulator to simulate the vehicle dispatching process. The DiDi operational dataset from November 2016 serves as the foundation for generating real-world data in this study.

Considering the high computational cost and impracticality of using Dijkstra’s algorithm to calculate distances for each instance, we simplify the model by calculating Manhattan distances when formulating the MIP. However, in the simulation process, Dijkstra’s algorithm is employed to simulate vehicle movement. Additionally, we assume that each order is associated with a single customer and that a vehicle can accommodate at most two passengers at a time.

\subsection{Objective Function}

The objective is to minimize the total distance between vehicles and passengers across all segments of the vehicle paths:
$$
\scalebox{0.85}{%
    \begin{minipage}{0.55\textwidth}
    \[
    \min \sum_{i=1}^{n_1} \sum_{j=1}^{m} x_{ij} \cdot d_{ij} + \sum_{i=1}^{n_1} \sum_{j=1}^{m} \sum_{k=1, k \neq j}^{m} y_{ijk} \cdot (d_{ij} + d_{jk}') + \sum_{i=1}^{n_2} \sum_{j=1}^{m} z_{ij} \cdot d_{ij}''
    \]
    \end{minipage}%
}
$$



 


where:

- \( x_{ij} \) is a decision variable indicating whether empty car \( i \) is assigned to user \( j \).

- \( y_{ijk} \) is a decision variable indicating whether empty car \( i \) is assigned to pick up user \( j \) and then user \( k \).

- \( z_{ij} \) is a decision variable indicating whether car \( i \) with one passenger willing to share is assigned to user \( j \).

- \( d_{ij} \) is the distance between vehicle \( i \) and user \( j \).

- \( d_{jk}' \) is the distance between user \( j \) and user \( k \).

- \( d_{ij}'' \) is the distance between vehicle \( i \) (with one order) and user \( j \).

\subsection{Constraints}
\label{sec:modeling:constraints}

1. Order Coverage: Each user is assigned to exactly one vehicle:
   \[
   \sum_i x_{ij} + \sum_i \sum_{k, j \neq k} (y_{ijk} + y_{ikj}) + \sum_{i'} z_{i',j} = 1, \ \forall \ j
   \]

2. Vehicle Capacity for Empty Vehicles: Each empty vehicle picks up at most two people:
   \[
   \sum_j x_{ij} + \sum_j \sum_{k \neq j} y_{ijk} \leq 1, \ \forall \ i
   \]

3. Vehicle Capacity for Shared Rides: Each vehicle with one passenger picks up at most one more person:
   \[
   \sum_j z_{ij} \leq 1, \ \forall \ i
   \]

4. Binary Variable Constraints:
   \[
   z_{i',j} \in \{0, 1\}, \ \forall \ i', j
   \]
   \[
   x_{ij} \in \{0, 1\}, \ \forall \ i, j
   \]
   \[
   y_{ijk} \in \{0, 1\}, \ \forall \ i, j, k
   \]
   
\subsection{Analysis of the Constraint Matrix}
As discussed in the \hyperref[sec:modeling:constraints]{constraints} section, Figure \ref{imgs:buildingModelTime} illustrates the relationship between the model-building time and the number of sets. As these numbers increase, the total number of constraints and variables grows, making the matrix larger and more complex. The shape of the constraint matrix is given by:
\[
(m+n+p, \; m \cdot p + m \cdot p^2 + n \cdot p)
\]

where:

-   m is the number of empty vehicles,

-   n is the number of vehicles with one order,

-   p is the number of orders.
% \begin{itemize}
%   \item \( m \) is the number of empty vehicles,
%   \item \( n \) is the number of vehicles with one order,
%   \item \( p \) is the number of orders.
% \end{itemize}




==> sections/4method.tex <==
\section{Method}
\label{sec:method}


\subsection{Data Collection and Prompt Generation}



\subsubsection{Data Storage}
When the simulator constructs and solves the MIP instances using the Gurobi solver, we capture several critical pieces of information that include (1) the location of every vehicle and order, (2) the status of intermediate feasible solutions, and (3) the optimal solution.



\subsubsection{Prompt Generation}

Following the collection of raw and intermediate data, we compile the LaTeX code for the model-building process, the details of each vehicle and order scenario, and both feasible and optimal solutions into a text format, as presented in \hyperref[sec:appendix]{Appendix}. This information is then used to generate the desired prompt for subsequent training and inference processes.

\subsection{Recursive CoT with dynamic temperature}

Since LLMs, after fine-tuning, exhibit a strong ability to grasp problem patterns, they often produce the same feasible solution at lower temperatures—even when the prompt suggests that this solution isn’t optimal. Despite recursive adjustments from lower temperatures to higher temperatures intended to explore a broader solution space, LLMs may still become trapped in the previous bad solutions. Thus, a temperature strategy is needed to effectively explore diverse possibilities and enhance solution quality.



To address this, we employ a recursive approach with dynamic temperature to leverage CoT effectively. Our strategy involves initially generating feasible solutions with a high temperature to explore a broader solution space. We then iteratively refine these solutions by gradually lowering the temperature. This dynamic temperature adjustment begins with a high temperature to facilitate exploration and progressively decreases to a low temperature to focus on refinement. This balanced approach helps us improve solution diversity and quality, ultimately leading to better feasible solutions.
